Bridging the Gap Between Foundation Models and Heterogeneous Federated Learning

Federated learning (FL) offers privacy-preserving decentralized machine learning, optimizing models at edge clients without sharing private data. Simultaneously, foundation models (FMs) have gained traction in the artificial intelligence (AI) community due to their exceptional performance across various tasks. However, integrating FMs into FL presents challenges, primarily due to their substantial size and intensive resource requirements. This is especially true when considering the resource heterogeneity in edge FL systems. We present an adaptive framework for Resource-aware Federated Foundation Models (RaFFM) to address these challenges. RaFFM introduces specialized model compression algorithms tailored for FL scenarios, such as salient parameter prioritization and high-performance subnetwork extraction. These algorithms enable dynamic scaling of given transformer-based FMs to fit heterogeneous resource constraints at the network edge during both FL's optimization and deployment stages. Experimental results demonstrate that RaFFM shows significant superiority in resource utilization efficiency and uses fewer resources to deploy FMs to FL. Despite the lower resource consumption, target models optimized by RaFFM achieve performance on par with traditional FL methods applied to full-sized FMs. This is evident across tasks in both natural language processing and computer vision domains.

==> content/02_droped_background.tex <==
\section{Background}
\subsection{Federated learning}
As concerns about user data privacy grow, there is an increasing need for AI models to be trained on decentralized data without sharing private information between clients. Federated Learning (FL) has emerged as a solution to this problem, offering a distributed and privacy-preserving machine learning approach that enables training on decentralized data without compromising data privacy~\cite{}.


In FL, raw data remains on local clients, ensuring data privacy and security while also enabling collaborative learning across multiple clients. The FL process involves local model training, model aggregation, and global model updates. Throughout this process, clients only share model updates, such as weights and gradients, asynchronously, reducing bandwidth requirements and minimizing the risk of data leaks and breaches.
A typical FL algorithm is FedAvg~\cite{}, which demonstrates the FL process (see Algorithm~\ref{algo:fedavg}). The privacy-preserving nature of FL has led to its widespread adoption in various applications, particularly in privacy-sensitive domains like healthcare.

\input{content/algorithm/fedavg}

However, FL still faces challenges related to heterogeneous data distribution. Data may be non-independent and identically distributed (non-IID) across clients, leading to poor model convergence and performance. Recent work in FL has focused on improving gradient descent to stabilize training~\cite{}; personalizing model weights to enhance performance on downstream tasks~\cite{}; and employing model compression techniques like knowledge distillation, dynamic dropout, and adaptive pruning to reduce overfitting on non-IID datasets and improve communication efficiency (Add specific examples of prominent works here).
(Add specific examples of prominent works here)

Despite these advances, there remains a gap between traditional model training and FL, particularly in terms of performance when dealing with heterogeneous data distributions.




\subsection{Foundation model}
Foundation Models (FMs) have emerged as a driving force in the field of AI, with large-scale pre-trained models such as GPT-3~\cite{}, GPT-4~\cite{}, ViT~\cite{}, CLIP~\cite{}, and BERT~\cite{} serving as the foundation for a wide variety of downstream tasks. These models are trained on massive amounts of data and have demonstrated remarkable capabilities across multiple domains. 
The lifespan of FMs usually includes pre-training, fine-tuning and transfer learning, and application.

First, the training process of FMs consists of two stages pre-training and fine-tuning in the lifespan of FMs. This two-stage process is crucial for the success of Foundation Models, as it enables them to learn general representations from large-scale datasets during pre-training and adapt to specialized tasks during fine-tuning. In the pre-training stage, which is usually an unsupervised or self-supervised learning process, models are trained on vast amounts of data. This is followed by the fine-tuning stage, where, given the broad knowledge FMs gain from the pre-training stage, they can be easily fine-tuned and transferred to specialized downstream tasks using supervised learning with labeled data.

For instance, Generative Pre-trained Transformer (GPT)~\cite{} is pre-trained on predicting the next word in a sequence given the context of the previous words in an unsupervised manner. During pre-training, GPT learns to generate text by completing sentences, which helps it capture grammar, syntax, semantics, and factual knowledge from the training data. This makes it easy to fine-tune GPT for a broad range of downstream tasks, such as text classification, sentiment analysis, translation, and summarization.



In application stage of FMs, 


\subsubsection{Newly Emerging Research in FMs}
One inspiring and charming of FMs is their extraordinary ability of adaptive to donwstream tasks with few-shot or even zero-shot learning. New research areas emerges to exploit such potential of FMs, such as Prompt Engineering, In-context Learning, etc.
In recent years, the AI research community has been actively exploring and developing novel techniques and strategies to leverage the full potential of foundation models. These emerging research areas seek to improve the adaptability, efficiency, and interpretability of FMs while reducing their reliance on extensive fine-tuning and labeled data. In this subsection, we will discuss some of the most promising and influential research directions in the field, including prompt engineering, zero-shot and few-shot learning, in-context learning, and continual/lifelong learning. By examining these cutting-edge advancements, we aim to provide a comprehensive understanding of the current state of the art in foundation model research and to highlight the immense opportunities that lie at the intersection of federated learning and foundation models.

\paragraph{Zero-Shot and Few-Shot Learning:} 
%1. brief introduce zero-shot and few-shot learning in FMs
%2. why FMs superior on zero and few shot learning
%3. examples on various of applications and use cases, also given the reference/
Zero-Shot and Few-Shot Learning are learning paradigms where models are required to adapt to new tasks without any labeled examples (zero-shot) or with very few labeled examples (few-shot). Foundation Models exhibit remarkable capabilities in these learning settings, allowing them to adapt to new tasks without or with very little task-specific training data. The superior performance of FMs in these paradigms can be attributed to the vast amounts of knowledge and general language understanding they acquire during the pre-training phase. FMs, such as CLIP~\cite{}, GPT-3~\cite{}, GPT-4~\cite{}, etc, have been proven that they can efficiently generalize to a wide range of applications and use cases, such as natural language understanding, machine translation, and sentiment analysis~\cite{}.
However, despite the remarkable success of FMs in zero-shot and few-shot learning, there are limitations and challenges to be addressed. For instance, the performance of FMs in these settings might be sensitive to the choice of prompts or task formulations, and they may struggle with tasks that require reasoning or knowledge outside their pre-training data. By investigating these challenges and exploring novel approaches, researchers aim to further enhance the adaptability and robustness of FMs in zero-shot and few-shot learning scenarios.







\paragraph{Prompt Engineering.} 
%1.what is prompt engineering
%2. why is important? (becasue we can get better performance)
%3. what kind of type we have? template, prompt tuning/insturction tuning
%4.give example and related work
Prompt Engineering is an emerging technology that focuses on optimizing the interaction between users and Foundation Models by carefully crafting and selecting prompts, thereby improving performance on downstream tasks. The significance of prompt engineering stems from its ability to fully exploit the potential of FMs and substantially enhance the accuracy and relevance of model responses, while minimizing the need for extensive fine-tuning.
Various methods for prompt engineering have been proposed. Prompt templates~\cite{} employ manually crafted and pre-defined linguistic patterns or structures to generate prompts. In contrast, prompt tuning~\cite{} and automated prompt generation~\cite{} involve training AI models or utilizing large language models to generate or discover high-quality prompts. Instruction tuning~\cite{}, a related method, is similar to prompt tuning but places greater emphasis on refining the model's understanding of natural language instructions embedded within the prompts. By fine-tuning the model on a dataset of input-output pairs, instruction tuning enhances the model's responsiveness and adaptability to a variety of tasks.

\paragraph{In-context Learning:} 
%1. briefly introduce what is in-context learning
%2. give related work and specific examples.
In-context Learning is a learning paradigm in which Foundation Models adapt to new tasks by leveraging the context provided within the input sequence itself. This approach allows FMs to learn from a series of examples or instructions, supplied as part of the input, without the need for explicit fine-tuning or labeled examples. In-context learning has been demonstrated to be effective in various applications, such as question-answering and programming tasks, with models like GPT-3 and GPT-4 showcasing impressive performance in these scenarios~\cite{}.
Recent work has explored different strategies for improving in-context learning, such as refining the input formatting or providing multiple examples within the context~\cite{}. One potential avenue for future research is the integration of in-context learning with federated learning in the context of Federated Foundation Models. This approach could enable models to learn from diverse, distributed data sources in a privacy-preserving manner, while still benefiting from the advantages of in-context learning. Investigating the combination of these techniques could lead to more robust and adaptable models that can efficiently learn from a wide range of data sources and contexts.

% \paragraph{Model compression:} Methods such as dropout, weight decay, and layer normalization can be employed to prevent overfitting and improve the generalization of Foundation Models. These techniques are important for mitigating the impact of non-IID data in Federated Learning, ensuring more robust and accurate models.


% Challenges and Limitations
% \subsubsection{Challenges and Limitations}
% Despite their remarkable success, Foundation Models present several challenges and limitations, including biases, ethical concerns, and the need for large-scale data and computation. Integrating Foundation Models with Federated Learning brings unique challenges, such as maintaining data privacy and dealing with non-IID data distributions. Research in this area aims to address these challenges and explore potential solutions to enhance the capabilities of Federated Foundation Models, paving the way for more robust, accurate, and privacy-preserving AI systems.

In summary, there are great opportunities in the intersection of FL and FM, 
which has the potential to revolutionize the AI landscape by leveraging the strengths of both paradigms. 
% Federated learning allows for decentralized and privacy-preserving data processing, enabling models to learn from a diverse range of data sources without violating user privacy. Meanwhile, foundation models excel at capturing rich representations and generalizing knowledge across a multitude of tasks. By integrating these two powerful approaches, we can create a new generation of AI systems that are not only more accurate and adaptive but also respectful of user privacy and data security.
This combination opens up numerous research directions and applications, ranging from personalized recommendations and natural language understanding to healthcare, finance, and beyond. As the AI research community continues to explore the intersection of federated learning and foundation models, we believe that a wide array of innovative solutions and breakthroughs will emerge, leading to more robust, efficient, and ethical AI systems that can better serve the needs of individuals and society as a whole.


%The Need for Federated Foundation Models

% \section{Foundation Models: A Brief Overview}
% \subsubsection{Definition and characteristics}
% Foundation Models~(FMs) are large-scale pre-trained machine learning models that serve as a starting point for downstream task-specific fine-tuning. These models, typically based on deep neural networks, capture a broad range of knowledge from diverse data sources and can be efficiently adapted to a wide array of tasks with minimal fine-tuning. 
% Key characteristics of foundation models include:

% \begin{itemize}
% \item Pre-training: Foundation models are trained on massive datasets to learn general-purpose features and representations.
% \item Transfer learning: These models can be fine-tuned with smaller labeled datasets for specific tasks, leading to improved performance and reduced training time.
% \item Multi-modal and multi-task capabilities: Foundation models can be designed to handle various data modalities (e.g., text, images, audio) and multiple tasks simultaneously.
% \end{itemize}

% \subsubsection{State-of-the-art foundation models}
% Transformer-based FMs have been developed in recent years and achieved state-of-the-art~(SoTA) performance in a wide range of scientific domains, particularly in natural language processing (NLP) and computer vision (CV). Some notable examples include:

% \begin{itemize}
% \item {BERT} (Bidirectional Encoder Representations from Transformers) \cite{devlin2018bert}: A transformer-based model that has achieved groundbreaking results in various NLP tasks, including question answering, sentiment analysis, and named entity recognition.
% \item {GPT} (Generative Pre-trained Transformer) \cite{radford2018improving}: Another transformer-based model initially designed for language modeling but has been successfully applied to a wide range of NLP tasks, with its latest version, GPT-3 \cite{brown2020language}, being one of the largest and most powerful language models available.

% % \item \textbf{ResNet} (Residual Networks) \cite{he2016deep}: A deep convolutional neural network (CNN) architecture for image recognition that introduced residual connections to alleviate the vanishing gradient problem, enabling the training of much deeper networks.

% \item {ViT} (Vision Transformer) \cite{dosovitskiy2020image}: A transformer-based model adapted for computer vision tasks, such as image classification and object detection, which demonstrates the potential of transformers to generalize beyond NLP tasks.
% \end{itemize}
% \subsubsection{Pre-training}
% Pre-training is the initial phase in the development of foundation models, where models are trained on large-scale datasets to learn general-purpose representations. This process involves unsupervised or self-supervised learning techniques, such as language modeling for natural language processing (NLP) tasks, or contrastive learning for computer vision tasks. Pre-training aims to: 
% Capture diverse knowledge and semantic structures from large-scale data sources.
% Learn transferable representations that can be efficiently adapted to downstream tasks.
% Reduce the need for extensive labeled data for task-specific fine-tuning.


% Recent advances in pre-training techniques have focused on improving efficiency, scalability, and transferability of foundation models \cite{liu2021gpt}. For example, methods like layer-wise learning rate adaptation \cite{you2020large} and model distillation \cite{hinton2015distilling} have been proposed to speed up the pre-training process and reduce computational requirements.

% \subsubsection{Fine-tuning and Transfer Learning}
% Once the foundation models are pre-trained, they can be fine-tuned on specific tasks using smaller labeled datasets. Fine-tuning involves updating the model's parameters through supervised learning to optimize performance on the target task. There are several approaches to fine-tuning, including instruction tuning and multi-task tuning:


%  \textbf{Instruction Tuning:} This approach involves training the model to understand and follow natural language instructions, allowing it to generalize across a range of tasks with minimal explicit supervision \cite{schick2021exploiting}. Instruction tuning typically requires modifying the model's input and output formats and adapting its loss function to the specific task.

%  \textbf{Multi-task Tuning:} In this approach, the foundation model is fine-tuned on multiple tasks simultaneously, which encourages the model to learn shared representations that generalize across tasks \cite{ruder2017overview}. Multi-task tuning can involve training the model on a combination of tasks with shared or separate task-specific layers, and may require designing novel training objectives and evaluation metrics to balance the trade-offs between tasks.

% \subsubsection{Prompting and Zero-shot Learning}
% Prompting and zero-shot learning are techniques that leverage the generalization capabilities of foundation models without requiring task-specific fine-tuning. These methods enable the models to perform new tasks by:

%  \textbf{Prompting:} Providing the model with a carefully designed input query or prompt, which guides the model to generate the desired output. This approach relies on the model's pre-trained knowledge and its ability to understand and respond to natural language instructions \cite{shin2020autoprompt}.
%  \textbf{Zero-shot Learning:} Training the model to recognize and classify novel instances or concepts without any prior exposure to labeled examples from those classes. Zero-shot learning often involves the use of auxiliary information, such as class descriptions or semantic embeddings, to bridge the gap between the pre-trained model and the target task \cite{soares2019matching}.

% \subsubsection{Challenges and limitations}
% Despite their remarkable performance, foundation models face several challenges and limitations, including:

% \begin{itemize}
% \item \textbf{Computational resources:} Training foundation models requires substantial computational power and energy, which may not be accessible to all researchers and organizations.

% \item \textbf{Data biases:} Foundation models can inherit biases present in their training data, which may lead to unintended consequences and ethical concerns when applied to real-world tasks \cite{bender2021dangers}.

% \item \textbf{Model interpretability:} Due to their complex nature, understanding the decision-making process of foundation models remains a challenge, limiting their applicability in safety-critical and regulated domains.

% \item \textbf{Adaptation to new tasks and domains:} While foundation models exhibit strong transfer learning capabilities, their performance may still be suboptimal for tasks or domains with limited available data or unique characteristics that deviate significantly from their pre-training data.
% \end{itemize}

% % \section{Background: Foundation Model Optimization}

% Foundation models have demonstrated remarkable performance across a wide range of tasks and domains. However, there is still room for improvement in terms of efficiency, generalization, and applicability. This section provides an overview of the key optimization strategies employed for foundation models, which include pre-training, fine-tuning, and prompting and zero-shot learning.




==> content/03_literature_review.tex <==
\section{Literature Review}
Overview of existing research on Federated Learning
Identification of gaps in the literature
Explanation of how the Federated Foundation Model fills these gaps
Comparison with other Federated Learning architectures

==> content/03_perspective.tex <==
\section{Motivation for Federated Foundation Models}
\label{sec:prospective}

In this section, we discuss the various challenges that motivate the development of Federated Foundation Models (FFMs), covering aspects such as data privacy, model performance, communication cost, scalability, deployment, personalization and real-time adaptation, and bias reduction. As shown in Figure~\ref{fig:FFM overview}, These existing challenges highlight the potential advantages of combining Foundation Models and Federated Learning for a wide range of applications and scenarios.


\textbf{Data privacy.}
The widespread deployment of AI in society generates vast amounts of data (e.g., images collected by cameras in smartphone applications), presenting potential resources for optimizing and specializing Foundation Models.
However, privacy concerns have limited the use of private data for FM optimization. 
FFMs offer significant improvements in data privacy by incorporating Federated Learning (FL), enabling FM optimization on private data. 
By optimizing FM tasks~(e.g., pre-training, fine-tuning, and prompt engineering) on local data without sharing raw information, FFMs comply with data protection regulations and preserve user privacy. This approach is particularly beneficial when sensitive data, such as medical records or personal communications, must be used to improve model performance without compromising confidentiality.


\textbf{Model performance.}
% Combining Foundation Models and Federated Learning offers mutual benefits that boost model performance. For Foundation Models, integrating Federated Learning allows access to a broader range of data for optimization tasks, such as prompt engineering, in-context learning, instruction tuning, fine-tuning, and pre-training. This expanded data access enables the development of more accurate and efficient AI systems that can better serve users in diverse scenarios.
% On the other hand, Federated Learning can also benefit from the integration of Foundation Models. FL typically suffers from the challenges of Non-IID and biased data, which may result in performance degradation for models trained under such conditions. However, Foundation Models contain comprehensive knowledge and can be easily specialized for various FL private tasks. By leveraging the advanced capabilities of Foundation Models, Federated Learning can overcome the limitations associated with Non-IID and biased data, leading to improved performance across different tasks and domains.
Combining FMs and FL provides benefits to FMs, boosting their performance. FMs gain access to a broader range of data for optimization tasks such as prompt engineering, in-context learning, instruction tuning, fine-tuning, and pre-training. This expanded data access enables the development of more accurate and efficient AI systems better suited for users in diverse scenarios. This combination benefits FL, as well. FL can overcome challenges associated with Non-IID~(Non-Identical Independent Distributed) and biased data by leveraging the advanced capabilities of Foundation Models, leading to improved performance across different tasks and domains.



\textbf{Cost.}
FFMs reduce communication costs by sharing only model updates between devices and the central server, significantly saving bandwidth and communication costs for transmitting raw data. Additionally, FFMs can potentially reduce the labor cost associated with collecting and managing data in a central location, as data is generated and used locally at edge devices. This efficiency makes FFMs a more practical and cost-effective solution for training and deploying FMs.




\textbf{Scalability.}
% Current FMs, especially large language models, often face scalability limitations due to the limited computational power at the edge. To mitigate these limitations, many Foundation Models are run centrally and provide API access for users. However, this approach can lead to capacity constraints and API congestion, hindering the widespread deployment of Foundation Models.
% In the near future, advancements in computational power available to users may enable Foundation Models to run locally on edge devices. The scalable nature of Federated Learning makes it an ideal framework for combining with Foundation Models, as it can accommodate numerous devices with varying computational capabilities. By integrating Federated Learning principles, Foundation Models can take advantage of these advancements in computational power and become more scalable, enabling broader deployment and improved performance across various tasks and domains.
Current FMs, especially large language models, often face scalability limitations due to limited computational power at the edge. Many FMs are run centrally and provide API access for users, which can lead to capacity constraints and API congestion. In the near future, advancements in computational power may enable FMs to run locally on edge devices. FL's scalable nature makes it an ideal framework for combining with FMs, accommodating numerous devices with varying computational capabilities. By integrating FL principles, FMs can leverage advancements in computational power, becoming more scalable and enabling broader deployment and improved performance across various tasks and domains.



\textbf{Deployment.}
% Federated Foundation Models offer potential advantages in terms of deployment, especially when it comes to reducing latency and enhancing user experience. When Foundation Models are run centrally and provide API access for users, latency can be an issue due to network communication between the user's device and the central server hosting the model. This latency can be affected by network conditions, server load, and other factors.
% In contrast, Federated Foundation Models can be deployed and run locally on edge devices, which has the potential to reduce latency by eliminating the need for network communication. This allows for faster response times and a more seamless user experience when interacting with the model.
% However, it is essential to consider the available computational resources on edge devices when deploying Foundation Models locally. As discussed in the Scalability section, advancements in computational power will be crucial for enabling the local deployment of Foundation Models on a wide range of devices, ensuring efficient and effective performance across various tasks and domains.
FFMs offer potential advantages in deployment, particularly in reducing latency and enhancing user experience. Running FMs centrally with API access for users can result in latency issues due to network communication between the user's device and the central server hosting the model. In contrast, FFMs can be deployed and run locally on edge devices, potentially reducing latency by eliminating network communication. This allows for faster response times and a more seamless user experience when interacting with the model. However, available computational resources on edge devices must be considered when deploying FMs locally. As discussed in the Scalability section, advancements in computational power will be crucial for enabling local deployment on a wide range of devices, ensuring efficient and effective performance across various tasks and domains.


\textbf{Personalization and real-time adaptation.}
FFMs facilitate a high degree of personalization by leveraging the decentralized nature of FL. By training on diverse, user-generated data, FMs can be tailored to individual preferences and requirements, offering more personalized and context-aware solutions across various tasks and domains.
A key advantage of FFMs is their ability to adapt in real-time as new personalized data becomes available from edge devices. This continuous learning capability ensures that the models remain up-to-date with users' evolving needs and preferences, further enhancing their personalization.
The focus on personalization in FFMs leads to improved performance and greater user satisfaction. By providing AI solutions that dynamically adapt to user-specific needs, FFMs enable more effective and engaging user experiences across a wide range of applications and domains.


% FFMs facilitate a high degree of personalization by leveraging the decentralized nature of FL. By training on diverse, user-generated data, FMs can be tailored to individual preferences and requirements, offering more personalized and context-aware solutions across various tasks and domains.
% One key advantage of Federated Foundation Models is their ability to adapt in real-time as new personalized data becomes available from edge devices. This continuous learning capability ensures that the models stay up-to-date with the evolving needs and preferences of users, further enhancing their personalization.
% The focus on personalization in Federated Foundation Models results in improved performance and greater satisfaction for users who interact with these models in their daily lives. By providing AI solutions that can dynamically adapt to user-specific needs, Federated Foundation Models enable more effective and engaging user experiences across a wide range of applications and domains.

\textbf{Bias reduction.}
% Federated Foundation Models contribute to bias reduction in AI systems by incorporating diverse data from decentralized sources, leading to more inclusive and fair AI solutions. The models learn from a wide variety of users and become more aware of the nuances and complexities of real-world scenarios, resulting in more informed and less biased decisions across tasks and domains.
% Moreover, the privacy-preserving nature of Federated Learning encourages more users to participate in the training process, further diversifying the data and knowledge incorporated into Foundation Models. This results in models better equipped to handle and minimize biases, providing fairer and more equitable AI solutions for all users.
FFMs contribute to bias reduction in AI systems by incorporating diverse data from decentralized sources, resulting in more inclusive and fair AI solutions. The models learn from various users, increasing their awareness of the nuances and complexities of real-world scenarios, and leading to more informed and less biased decisions across tasks and domains.
Additionally, the privacy-preserving nature of FL encourages more users to participate in the training process, further diversifying the data and knowledge incorporated into FMs. This results in models better equipped to handle and minimize biases, providing fairer and more equitable AI solutions for all users.

\textbf{Continual/Lifelong learning.} 
% Continual or Lifelong Learning refers to the ability of AI models to learn and adapt to new tasks and information over time without forgetting previously acquired knowledge. This learning paradigm aims to mimic human learning, which is characterized by the continuous accumulation and integration of knowledge throughout an individual's lifetime. The benefits of continual/lifelong learning include better generalization across tasks, efficient transfer learning, and more robust adaptation to new and changing environments~\cite{}.
% Recent research in the field of continual/lifelong learning has focused on techniques such as experience replay, elastic weight consolidation, and meta-learning, which enable models to maintain and update their knowledge efficiently~\cite{}. Integrating these approaches with Foundation Models could unlock new opportunities for developing more versatile and adaptive AI systems. In the context of Federated Foundation Models, continual/lifelong learning could be particularly beneficial as it enables models to learn from diverse and distributed data sources continuously while preserving privacy. Exploring the combination of federated learning and continual/lifelong learning could lead to the development of advanced AI models that can effectively leverage distributed data while adapting to new tasks and challenges throughout their lifespan.
FMs combined with FL provide an ideal platform for continual lifelong learning. This combination facilitates the continuous adaptation and improvement of models by harnessing decentralized and diverse data sources, leading to more versatile and effective AI systems. As advancements in edge computing power become more prevalent, the realization of continual lifelong learning in Foundation Models will soon be within reach. This progress will enable AI models to learn and grow throughout their lifespan, unlocking new possibilities for AI research and practical applications in various domains. By embracing continual lifelong learning, FFMs can help create more adaptive, efficient, and personalized AI systems that can dynamically adjust to user-specific needs and preferences, ultimately benefiting users from all walks of life.







In summary, FFMs offer a promising approach to address many challenges and limitations associated with traditional, centralized machine learning. By integrating FL into FM optimization, we can create more efficient, personalized, privacy-preserving, and inclusive AI systems. This opens up new possibilities for AI research and practical applications, making AI more accessible and beneficial to users from all walks of life.










==> content/04_federated_FM.tex <==
\input{content/f02_ffm_tasks}
\section{Federated Foundation Models}
In this section, we introduce and discuss potential tasks and applications related to Federated Foundation Models~(FFMs), including:
\begin{itemize}
\item Federated Foundation Model Pre-training
\item Federated Foundation Model Fine-tuning
\item Federated Prompt Engineering
\item Federated Continual (Lifelong) Learning
\end{itemize}
We examine the unique characteristics and requirements of these tasks, highlighting the opportunities and challenges that arise when leveraging FFMs to tackle real-world problems. Our goal is to establish a solid foundation for understanding the scope and potential of this new paradigm, paving the way for future research and development. As mentioned in Section~\ref{sec:prospective}, some tasks may not be feasible until computational power at the edge advances further.

\subsection{Federated Foundation Model Pre-training}
% The motivation for FFM pre-training is not to replace traditional FM pre-training methods but to enhance them by applying FL's ability to leverage private data for improved model generalizability while maintaining data privacy. By utilizing private data, the model can access a wider range of knowledge, reduce the risk of overfitting public data, and potentially enable more personalized and context-aware models, all while the FM can still learn from well-crafted centralized data.
Federated Foundation Model pre-training~(FFM pre-training) aims to enhance traditional FM pre-training methods by incorporating Federated Learning's~(FL's) ability to leverage private data for improved model generalization while maintaining data privacy. This allows the model to access a wider range of knowledge, reduce overfitting on public data, and potentially enable more personalized and context-aware models, while still benefiting from centralized data.


The FFM pre-training process involves two stages: centralized pre-training on public data and federated pre-training on private data. As shown in Figure~\ref{fig:FFM_tasks}, these stages interact through an adaptive switching mechanism, allowing the model to alternate between centralized pre-training and federated pre-training.
For example, an FFM pre-training round may involve pre-training the model on public data for $n_c$ epochs using existing FM pre-training methods, followed by pre-training for $n_f$ epochs on private data via federated learning. The FFM can also first pre-train via FL and then on centralized public data, providing a flexible and adaptive process. Existing federated learning algorithms can be adapted for FM pre-training to enable seamless integration of federated learning benefits.

The main advantage of FFM pre-training is its flexibility, as it builds on existing FM pre-training methods without extensive modifications. This approach can easily incorporate future advancements in FM pre-training while maintaining the benefits of both existing methods and federated learning. However, it is crucial to consider the available computational resources on edge devices when deploying Foundation Models locally. Advancements in computational power will be essential for enabling local deployment on a wide range of devices, ensuring efficient performance across various tasks and domains.
% The Federated Foundation Model Pre-training methodology builds on top of existing FM pre-training methods and integrates federated learning into the process. As shown in Figure~\ref{} and Algorithm~\ref{}, the Federated Foundation Model pre-training process can be described as the interaction of two types of training: centralized pre-training on public data and federated pre-training on private data. These two stages of pre-training interact with each other through the Federated Foundation Model pre-training process, where the FM adaptively switches between centralized pre-training on public data and federated pre-training on distributed private data.

% For instance, a Federated Foundation Model pre-training round can be formulated as follows: the FM is first pre-trained on public data for $n_c$ epochs via existing FM pre-training methods, and then pre-trained for $n_f$ epochs on private data using federated learning. Alternatively, the Federated Foundation Model is highly flexible and adaptive, allowing for the possibility to pre-train via FL first, then pre-train on centralized public data. To achieve this, existing federated learning algorithms can be adapted for Foundation Model pre-training, allowing for a seamless integration of federated learning benefits into the pre-training process.

% One of the main advantages of Federated Foundation Model Pre-training is its flexibility. As it builds on top of existing FM pre-training methods without extensive modifications, this approach can easily incorporate future advancements in FM pre-training while maintaining the benefits of both existing FM pre-training methods and federated learning. This flexibility allows for a more robust and adaptable pre-training process, resulting in models that are better suited for a wide range of tasks and applications.

% Again, it is essential to consider the available computational resources on edge devices when deploying Foundation Models locally. As discussed in the Scalability section, advancements in computational power will be crucial for enabling the local deployment of Foundation Models on a wide range of devices, ensuring efficient and effective performance across various tasks and domains.
% Explanation of the Federated Foundation Model and its components
% Technical details of implementing the Federated Foundation Model
% Evaluation metrics and criteria for success

%benefit of federated FM fine-tuning vs simply deploy and personalized FMs.
\subsection{Federated Foundation Model Fine-tuning}
Traditional FM fine-tuning often involves offline deployment, where the model is fine-tuned on private data and then isolated, preventing collaboration between end-users. This approach may not fully exploit the potential of the FM, especially when local private data is limited or biased.
Federated Foundation Model fine-tuning (FFM fine-tuning) addresses these limitations by fostering collaboration between end-users while preserving data privacy. This approach allows for direct fine-tuning of FMs on private data at the edge for downstream tasks while sharing the fine-tuned FMs with other clients/end-users, enabling a more robust and better-performing model.

As shown in Figure~\ref{fig:FFM_tasks}, FFM fine-tuning builds upon FFM pre-training and employs an adaptive switching mechanism that alternates between centralized fine-tuning on public datasets for benchmark tasks and federated fine-tuning on private data with local tasks. We propose two FFM fine-tuning strategies: (1) directly fine-tuning the FM backbone, and (2) fine-tuning a lightweight adapter head while keeping the FM backbone frozen.

In the first strategy, the FM backbone's weights are updated on user private data and evaluated on local tasks, then uploaded to the server for aggregation across all clients. The server also leverages public data to fine-tune the aggregated FM on benchmark tasks. However, the complexity of FMs can make this strategy difficult to apply at the edge right now, particularly in resource-limited scenarios.

To address this challenge, we propose the second strategy of fine-tuning a lightweight adapter head while keeping the FM backbone frozen. This approach uses an adapter to transfer the FM's capabilities directly to local tasks, sharing only the lightweight adapter between the edge and the server. This improves efficiency in both computation and communication while maintaining the benefits of FFM fine-tuning. Moreover, due to the scalability and heterogeneity of FL, FFM fine-tuning can be easily extended to multi-modal tasks.

In summary, FFM fine-tuning provides a promising alternative to traditional FM fine-tuning, offering increased privacy, collaboration, adaptability, and efficiency. This approach has the potential to improve both the performance and generalizability of Foundation Models across various applications and domains.















% Similar to Federated Foundation Model Pre-training, the Federated Foundation Model fine-tuning methodology builds upon traditional federated learning approaches. It deploys the FM at edge institutions and fine-tunes the FM on private data at the edge. Within the fine-tuning process, the participate institutions can share their fine-tuned model to aggregate to a more generalized global model.

% One of the benefits of federated fine-tuning is that it enables collaboration with other private institutions that have similar downstream tasks, allowing for more efficient fine-tuning through shared knowledge and expertise.
% Another key advantage of Federated Foundation Model fine-tuning is the enhanced privacy it offers, as private data never leaves the edge institutions. Furthermore, the adaptability of the Federated Foundation Model fine-tuning methodology allows it to be tailored to different edge institutions and their specific downstream tasks, leading to more personalized and context-aware models.

% Overall, Federated Foundation Model fine-tuning offers a promising alternative to traditional FM fine-tuning, with increased privacy, collaboration, adaptability, and efficiency. This approach has the potential to improve both the performance and generalizability of Foundation Models across a wide range of applications and domains.

\subsection{Federated prompt engineering}
Integrating FL into prompt engineering has promising potential for enhancing the performance of FMs while preserving data privacy. For instance, FFMs can enable the use of sensitive data in prompt templates, allowing more accurate and personalized prompt conditioning for tasks like in-context learning. By providing contextual priors or examples from private data, the model can better understand and generate context-aware responses while ensuring the sensitive data never leaves the local end-user.

Here we mainly discuss the automated prompt (soft prompt) methods, such as instruction tuning~\cite{wei2021prompt}, which refines the model's understanding of natural language instructions, and prompt tuning~\cite{lester2021prompt_tune}, which tailors the input prompt to improve the model's output. As shown in Figure~\ref{fig:FFM_tasks}, in federated prompt engineering settings, 
In federated prompt engineering settings, end-users can collaboratively train auto prompt models (prompt generator components in Figure~\ref{fig:FFM_tasks}) on their local private data and tasks, sharing the learned auto prompt models without exposing the sensitive data. 
This collaborative process allows for the creation of more effective and adaptable prompts, improving the overall performance of Foundation Models on downstream tasks.

Federated prompt engineering not only facilitates the development of better prompts using private data but also maintains the privacy of sensitive information. By combining the advantages of FL with the power of FMs, federated prompt engineering opens up new possibilities for the deployment of AI systems across various domains and applications.









\subsection{Federated continual (lifelong) learning}
One disadvantage of FMs is their limitation to pre-trained, offline knowledge. For example, ChatGPT's knowledge is up-to-date only until 2021. With the anticipated increase in computational power, FM optimization at the edge may become feasible. FFMs can unlock the possibility of continual/lifelong learning from newly generated private edge data. With its scalability and privacy-preserving nature, FL can harness decentralized power to optimize FMs using emerging private data at the edge, which can serve as a valuable resource for model optimization.

In terms of methodology, a federated server can be established to facilitate communication between the server and edge end-users. The Foundation Model is optimized at the edge, with local updates sent to the server for aggregation. This process keeps the global model up-to-date while preserving data privacy, as local private data remains at the edge and is never directly shared. The server then sends the updated global model back to the edge institutions or clients, ensuring that each participant benefits from the collaborative learning process.

Moreover, federated continual/lifelong learning can contribute to more efficient use of resources, as institutions no longer need to retrain their models from scratch whenever new data becomes available. By leveraging federated learning, institutions can incrementally improve their models, reducing the time and computational resources required for model training and refinement.

One additional point to consider is the adaptability of Federated Continual/Lifelong Learning to handle non-stationary data distributions. As the world is constantly changing, data distributions may shift over time. This approach enables the continual adaptation of FMs to ever-changing real-world scenarios, enhancing their performance in dynamic environments.








==> content/06_challenges_future.tex <==
\section{Conclusion and discussion}

In this paper, we introduced the concept of Federated Foundation Models (FFMs), which integrate Federated Learning (FL) into the lifespan of Foundation Models (FMs). We defined three FFM tasks: FFM pre-training, FFM fine-tuning, and federated prompt engineering. Through our experiments, we demonstrated that FFM can significantly improve the performance of centralized FM optimization by leveraging local private data, and the flexible and adaptive optimization process between centralized training and FL makes it more stable and robust than FL-only optimization.

It is important to note that the advancement of computation at edge users is crucial for the widespread adoption of FFMs, and we believe that such advancements will be realized in the near future. As the field of FFM continues to grow, we anticipate the emergence of numerous related research areas, including improved privacy-preserving techniques, the integration of FFM with emerging technologies like IoT and edge computing, and the exploration of FFM in various application domains such as healthcare, finance, and manufacturing.
Additionally, we foresee advancements in adaptive model compression methods for FFM local institutions, communication efficiency research, specialized FL algorithms for efficient updates and aggregation of FFM models, and security attack research. Overall, FFM represents a promising research area in the age of Foundation Models, with the potential to address various challenges in privacy, scalability, and robustness across diverse domains.








==> content/10_proof.tex <==
\appendix
\section{Appendix}
You may include other additional sections here.

\textbf{Salient Parameter Prioritization.} 
We ranking the original model weights channels based on the salience score for better subnetwork extraction and model fusion in FL global updates. Prioritization ensures that the most impactful channels are at forefront of the weight matrix:
    \begin{equation}
    c_{ranked} = \text{argsort}(\text{Salience}(c), \text{descending})
    \label{eq:channel_order}
    \end{equation}
    \begin{equation}
    W_{ranked} = W[c_{ranked}:]
    \label{eq:channel_order}
    \end{equation}
    Equation \ref{eq:channel_order} describes the process of ordering channels based on their computed salient score.

 \subsubsection{Parameter Prioritization in Transformer}
Existing magnitude-based compression methods mainly focus on convolution neural networks (CNNs), transformer~\cite{}, with their multi-head attention mechanisms, need further consideration. We proposed specialized salient parameter prioritization for multi-head transformers.

\begin{equation}
\label{eq:multihead}
\text{Attention}(W^q,W^k,W^v,x) = \text{softmax}\left(\frac{xW^q (xW^k)^T}{\sqrt{d_k}}\right) xW^v
\end{equation}

We can simplify the computation as Equation~\ref{eq:multihead}, where the input sequence $x\in \mathcal{R}^{n\times d}$ with sequence length $n$ and embedding size $d$, $W^q \in \mathcal{R}^{d\times d_k}$ and $W^k \in \mathcal{R}^{d\times d_k}$ are the query and key weights, and $W^v \in \mathcal{R}^{d\times d_v}$ is the value weights.

To satisfy the Rule~\ref{itm:rule2}, in transformer architecture, we only prioritize the $W^q$ and $W^k$.  Specifically, we compute the average norm for the query (q) and key (k) matrices in each channel. 
We decompose $W^q$ and $W^k$ as a set of vectors:
$W^q = [w^q_1, ...,w^q_c,..., w^q_{d_k}]$ and $W^k = [w^k_1, ...,w^k_c,..., w^k_{d_k}]$, where $w^q_c \text{,  } w^k_c \in\mathcal{R}^{d\times1}$, and $c \in [1,d_k]$.
% $$ W^k = {w^k_c} \text{,    \space} c \in [1,d_k] $$

Importantly, an identical ranked order is applied to $W^q$ and $W^k$ together. Formally, in attention layers, for a given channel $c$ in $W^q$ and $W^k$ we calculate the average L1 norm as salient parameter score as Equation~\ref{eq:avg_norm}.
     % \text{AvgNorm}(c) = \frac{\text{Norm}(q_c) + \text{Norm}(k_c) + \text{Norm}(v_c)}{3}
    \begin{equation}
    \text{Norm}(c) = \frac{\text{Norm}(w^q_c) + \text{Norm}(w^k_c) }{2}
    \label{eq:avg_norm}
    \end{equation}
The average norm provides a unified measure for the attention mechanism, then we ensure that all components $(W^q, W^k)$ are consistently ranked with the same permutation $\pi$ in Equation~\ref{eq:argsort}~\ref{eq:wq'}~\ref{eq:wk'}.

\begin{equation}
 \pi = \text{argsort}(\text{Norm}(1),\ldots, \text{Norm}(c), \ldots, \text{Norm}({d_k})) 
 \label{eq:argsort}
\end{equation}

\begin{equation}
W^{q'} = [w^q_{\pi(1)}, ..., w^q_{\pi(d_k)}] 
\label{eq:wq'}
\end{equation}


\begin{equation}
W^{k'} = [w^k_{\pi(1)}, ..., w^k_{\pi(d_k)}]
\label{eq:wk'}
\end{equation}


 % Consider a simple FM with three channels, where the L1 norms of the weights for these channels are 10, 15, and 5, respectively. Using our method, the channels would be ranked in the order: 2, 1, 3, indicating the importance of each channel based on its weight magnitude.



\textbf{Theorem}: Given matrices $W^q$ and $W^k$ of size $d \times d_k$ and an input $x$ of size $n \times d$, if we apply a consistent permutation $\pi$ to the columns of both $W^q$ and $W^k$ to obtain $W^{q'}$ and $W^{k'}$, respectively, then the resulting dot-product attention scores computed using $W^{q'}$ and $W^{k'}$ will be identical to those computed using the original $W^q$ and $W^k$.

\textbf{Proof}:

Let $Q = xW^q$ and $K = xW^k$ be the original query and key matrices. Their sizes are $n \times d_k$.

Let $Q' = xW^{q'}$ and $K' = xW^{k'}$ be the query and key matrices after applying the permutation $\pi$. 

By our definition of the permutation, for each column $c$ in $W^q$ and $W^k$, the new position in the permuted matrices is $\pi(c)$. So, the elements of $Q'$ and $K'$ are given by:
\begin{equation}
    Q'_{ij} = \sum_{c=1}^{d} x_{ic} W^{q'}_{cj} = \sum_{c=1}^{d} x_{ic} W^{q}_{c\pi(j)} = x_i \cdot \Vec{w}^q_{\pi(j)}
    \label{eq:Q'}
\end{equation}
\begin{equation}
    K'_{ij} =  \sum_{c=1}^{d} x_{ic} W^{k'}_{cj} = \sum_{c=1}^{d} x_{ic} W^{k}_{c\pi(j)} = x_i \cdot \Vec{w}^k_{\pi(j)}
    \label{eq:K'}
\end{equation}


Now, consider the dot-product of rows from $Q$ and $K$:
\begin{equation}
    (QK^T)_{ij} = \sum_{c=1}^{d_k} Q_{ic} K_{jc} 
\end{equation}


Similarly, for $Q'$ and $K'$:
\begin{equation}
    (Q'K'^T)_{ij} = \sum_{c=1}^{d_k} Q'_{ic} K'_{jc}
\end{equation}


Using the previous definitions of $Q'$ and $K'$, and plugging them into the above equation, we see:
\begin{equation}
\begin{split}
\label{eq:Q'K'}
(Q'K'^T)_{ij} & = \sum_{p=1}^{d_k} \left( \sum_{c=1}^{d} x_{ic} W^{q'}_{cp} \right) \left( \sum_{r=1}^{d} x_{jr} W^{k'}_{rp} \right) 
\end{split}
\end{equation}

We take the Equation~\ref{eq:Q'}~\ref{eq:K'} into Equation~\ref{eq:Q'K'} and we have:
\begin{equation}\label{eq:Q'K'=QK}
\begin{split}
       (Q'K'^T)_{ij}  &= \sum_{p=1}^{d_k} \left( x_i \cdot \Vec{w}^q_{\pi(p)} \right) \left( x_j \cdot \Vec{w}^k_{\pi(p)} \right) 
       \\ &= \sum_{p=1}^{d_k} \left( x_i \cdot \Vec{w}^q_{p} \right) \left( x_j \cdot \Vec{w}^k_{p} \right) 
\end{split}
\end{equation}

Because the permutation $\pi$ is applied consistently to both $W^q$ and $W^k$, and the dot product operation is commutative, each term of the form $x_{i} \cdot W^{q'}_{\pi(p)}$ will correspond to a term of the form $x_{j} \cdot W^{k'}_{\pi(p)}$, yielding identical products as in the original $QK^T$ computation.

Therefore, we can conclude that:
\[ QK^T = Q'K'^T \]

Hence, the attention scores remain unchanged after the permutation.


==> content/f02_glue.tex <==
\begin{figure}
  \centering
  \includegraphics[width=.5\linewidth]{content/figures/glue_imag.pdf}
    % \includegraphics[width=.5\linewidth]{content/figures/squad_param_efficiency.pdf}

  \caption{result on GLUE}
  \label{fig:glue_res}
\end{figure}


==> content/f04_communication_footprint.tex <==
\begin{figure}
  \centering
  \includegraphics[width=.3\linewidth]{content/figures/com_footprint.pdf}
  \caption{The average communication footprint in each communication round.}
  \label{fig:com_footprint}
\end{figure}


==> content/t04_method_compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Experiments on question answering tasks}
\label{tab:fl_compare}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|cccc|cccc|}
\hline
\multirow{4}{*}{\textbf{}}                                                    & \multirow{2}{*}{\textbf{Federated Learning}} & \multicolumn{4}{c|}{\multirow{2}{*}{\textbf{Efficient Finetuning}}}                                               & \multicolumn{4}{c|}{\multirow{2}{*}{\textbf{Resource-aware FL}}}                                                  \\
                                                                              &                                              & \multicolumn{4}{c|}{}                                                                                             & \multicolumn{4}{c|}{}                                                                                             \\
                                                                              & \multirow{2}{*}{\textbf{}}                   & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{}} \\
                                                                              &                                              &                            &                            &                            &                            &                            &                            &                            &                            \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Communication\\ Cost\end{tabular}} & \multirow{2}{*}{4TB}                         & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          \\
                                                                              &                                              &                            &                            &                            &                            &                            &                            &                            &                            \\ \hline
\multirow{2}{*}{Training Cost}                                                & \multirow{2}{*}{}                            & \multicolumn{4}{c|}{\multirow{2}{*}{}}                                                                            & \multicolumn{4}{c|}{\multirow{2}{*}{}}                                                                            \\
                                                                              &                                              & \multicolumn{4}{c|}{}                                                                                             & \multicolumn{4}{c|}{}                                                                                             \\ \hline
\multirow{2}{*}{Memory}                                                       & \multirow{2}{*}{12GB For every Client}       & \multicolumn{4}{c|}{\multirow{2}{*}{12GB +1GB For every Client}}                                                  & \multicolumn{4}{c|}{\multirow{2}{*}{2-12GB}}                                                                      \\
                                                                              &                                              & \multicolumn{4}{c|}{}                                                                                             & \multicolumn{4}{c|}{}                                                                                             \\ \hline
\multirow{2}{*}{Storage}                                                      & \multirow{2}{*}{6 GB}                        & \multirow{2}{*}{7GB}       & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{0.5-6GB}   & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          \\
                                                                              &                                              &                            &                            &                            &                            &                            &                            &                            &                            \\ \hline
\multirow{2}{*}{Inference}                                                    & \multirow{2}{*}{20ms}                        & \multirow{2}{*}{24ms}      & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{5ms}       & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          \\
                                                                              &                                              &                            &                            &                            &                            &                            &                            &                            &                            \\ \hline
\multirow{2}{*}{Performance}                                                  & \multirow{2}{*}{}                            & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{}          \\
                                                                              &                                              &                            &                            &                            &                            &                            &                            &                            &                            \\ \hline
\end{tabular}%
}
\end{table}

==> content/t05a.com_target.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

\begin{table}[t]
\caption{Communication cost for achieving target performance on QA benchmark}
\label{tab:com_cost}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}}                       & \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Edge\\ Resource Usage\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Target Performance\\ (F1 Score)\end{tabular}}} & \multicolumn{3}{c}{\textbf{Communication Cost}}                   & \textbf{}         \\
                                &                                                        &                                   &                                                                                         &                                                                                                   & \textbf{Traffic/Client} & \textbf{Total} & \textbf{$\Delta$ Cost} & \textbf{Speed Up} \\ \hline
\multirow{4}{*}{BERT-Large}     & FL                                                     & \multirow{2}{*}{SQUADv1}          & 334M                                                                                    & \multirow{2}{*}{85\%}                                                                             & 1401MB                  & 109.45GB       & -                      &                   \\
                                & \begin{tabular}[c]{@{}c@{}}RaFFM\\ (Ours)\end{tabular} &                                   & 95M                                                                                     &                                                                                                   & 398MB                   & 46.64GB        & -62.81GB               &                   \\
                                & FL                                                     & \multirow{2}{*}{SUQADv2}          & 335M                                                                                    & \multirow{2}{*}{90.09\%}                                                                          & 1401MB                  & 73.88 GB       & -                      &                   \\
                                & \begin{tabular}[c]{@{}c@{}}RaFFM\\ (Ours)\end{tabular} &                                   & 103M                                                                                    &                                                                                                   & 432MB                   & 24.47 GB       & 49.41 GB               &                   \\ \hline
\multirow{4}{*}{BERT-Base}      & FL                                                     & \multirow{2}{*}{SQUADv1}          & 109M                                                                                    & \multirow{2}{*}{80.42\%}                                                                          & 457.38MB                & 223.33GB       &                        &                   \\
                                & \begin{tabular}[c]{@{}c@{}}RaFFM\\ (Ours)\end{tabular} &                                   & 70M                                                                                     &                                                                                                   & 293.73MB                & 177.84GB       &                        &                   \\
                                & FL                                                     & \multirow{2}{*}{SQUADv2}          & 109M                                                                                    & \multirow{2}{*}{76.21\%}                                                                          & 457.38MB                & 196.53GB       &                        &                   \\
                                & \begin{tabular}[c]{@{}c@{}}RaFFM\\ (Ours)\end{tabular} &                                   & 73M                                                                                     &                                                                                                   & 306.32MB                & 221.36GB       &                        &                   \\ \hline
\multirow{4}{*}{DistillBERT}    & FL                                                     & \multirow{2}{*}{SQUADv1}          & 67M                                                                                     & \multirow{2}{*}{80.15\%}                                                                          & 281.14MB                & 29.65 GB       &                        &                   \\
                                & \begin{tabular}[c]{@{}c@{}}RaFFM\\ (Ours)\end{tabular} &                                   & 34M                                                                                     &                                                                                                   & 142.67MB                & 27.31 GB       & 2.34 GB                &                   \\
                                & FL                                                     & \multirow{2}{*}{SQUADv2}          & 67M                                                                                     & \multirow{2}{*}{79.55\%}                                                                          & 281.14MB                & 50.52 GB       &                        &                   \\
                                & \begin{tabular}[c]{@{}c@{}}RaFFM\\ (Ours)\end{tabular} &                                   & 34M                                                                                     &                                                                                                   & 142.67MB                & 25.64 GB       & -24.88 GB              &                   \\ \hline
\multirow{4}{*}{RoBERTa}        & FL                                                     & \multirow{2}{*}{SQUADv1}          & 124M                                                                                    & \multirow{2}{*}{86.68\%}                                                                          & 520.32MB                & 152.44GB       &                        &                   \\
                                & \begin{tabular}[c]{@{}c@{}}RaFFM\\ (Ours)\end{tabular} &                                   & 90M                                                                                     &                                                                                                   & 377.66MB                & 132.77GB       &                        &                   \\
                                & FL                                                     & \multirow{2}{*}{SQUADv2}          & 124M                                                                                    & 85.29\%                                                                                           & 520.32MB                & 152.43GB       &                        &                   \\
                                & \begin{tabular}[c]{@{}c@{}}RaFFM\\ (Ours)\end{tabular} &                                   & 89M                                                                                     &                                                                                                   & 373.46MB                & 124.00GB       &                        &                   \\ \hline
\end{tabular}%
}
\end{table}
